Design2Cloth: 3D Cloth Generation from 2D Masks

In recent years, there has been a significant shift in the field of digital avatar research, towards modeling, animating and reconstructing clothed human representations, as a key step towards creating realistic avatars. However, current 3D cloth generation methods are garment specific or trained completely on synthetic data, hence lacking fine details and realism. In this work, we make a step towards automatic realistic garment design and propose Design2Cloth, a high fidelity 3D generative model trained on a real world dataset from more than 2000 subject scans. To provide vital contribution to the fashion industry, we developed a user-friendly adversarial model capable of generating diverse and detailed clothes simply by drawing a 2D cloth mask. Under a series of both qualitative and quantitative experiments, we showcase that Design2Cloth outperforms current state-of-the-art cloth generative models by a large margin. In addition to the generative properties of our network, we showcase that the proposed method can be used to achieve high quality reconstructions from single in-the-wild images and 3D scans. Dataset, code and pre-trained model will become publicly available.

==> sec/table_large.tex <==

\newcolumntype{g}{>{\columncolor{Gray}}c}
\begin{table*}
\begin{center}
\scalebox{0.71}{
\begin{tabular}{l c c c c c c c c c c}
\hline

Method & 
        Dataset &\#Garment & \#Subjects & \#Categories & Real Data & Cloth design & Generation & 
        Garment-Generic &Animation & Animation Losses  \\
\hline

DRAPE\cite{guan2012drape} & \checkmark & 420 & 420 & 5 & $\times$ & $\times$ & \checkmark & $\times$ & \checkmark &  Learn from PCA \\


DeepGarment~\cite{danvevrek2017deepgarment} &\checkmark & 
        2 & 10 & 2 & $\times$ & $\times$ &\checkmark & 
        $\times$ & $\times$ &  - \\



Wang et al\cite{wang2018learning} & \checkmark & 8k & - & 3 & $\times$ & \checkmark & \checkmark &$\times$ & $\times$ &  - \\

% 3DPeople\cite{Pumarola_2019_ICCV} & \checkmark & - & 80 & - & $\times$ & $\times$ & \checkmark & \checkmark & $\times$ &  - \\



Santesteban et al.\cite{santesteban2019learning} & \checkmark & 17 & 17 & 1 & $\times$ & $\times$ & \checkmark & $\times$ & \checkmark &  Displacement loss \\

GarNet\cite{Gundogdu_2019_ICCV} & \checkmark & 1.5k & 500 & 3 & $\times$ & $\times$ & \checkmark & $\times$ & \checkmark &  L2 loss+physics-based \\


TailorNet\cite{Patel_2020_CVPR} & \checkmark & 207 & 9 & 4 & $\times$ & $\times$ & \checkmark &$\times$ & \checkmark &  L1 loss \\

Cloth3D\cite{bertiche2020cloth3d} & \checkmark & 11.3K & 8.5k & 7+ & $\times$ & $\times$ & \checkmark & \checkmark & $\times$ &  - \\


Shen et al.\cite{shen2020gan} & \checkmark & 100+ & - & 5 & $\times$ & \checkmark & \checkmark & \checkmark & $\times$ &  - \\

SMPLicit\cite{corona2021smplicit} & \checkmark & 2705k+ & - & 11 & $\times$ & $\times$ & \checkmark & \checkmark & $\times$ &  - \\

DIG\cite{Li_2022_ACCV} & $\times$ &200 &- &2 & $\times$ & $\times$ & \checkmark & \checkmark & \checkmark &  L1 loss \\

DrapeNet~\cite{De_Luigi_2023_CVPR} &\times  &
        900 & - & 5 & $\times$ & $\times$ & \checkmark & 
        \checkmark & \checkmark &  physics-based \\

HOOD~\cite{Grigorev_2023_CVPR} &\times & 
        15 & - & 7 & \times & $\times$ & \times & 
        \checkmark & \checkmark &   physics-based\\

Zhao et al.~\cite{Zhao_2023_CVPR} &\times & 
        2 & - & 2 & \times & $\times$ & \times & 
        \times & \checkmark &  L2 loss+L_{reg} \\

CLOTH4D\cite{Zou_2023_CVPR} & \checkmark & 1k & 1k & 6 & $\times$ & $\times$ & $\times$ & - & $\times$ &  - \\

ClothesNet\cite{zhou2023clothesnet} & \checkmark & 4.4k & - & 11 & $\times$ & $\times$ & $\times$ & - & $\times$ &  - \\


\rowcolor{grey}
BUFF\cite{Zhang_2017_CVPR} & \checkmark & 24 &6 &4 & \checkmark & $\times$ & $\times$ & \checkmark & $\times$ & - \\

\rowcolor{grey}
ClothCap~\cite{pons2017clothcap} &$\times$ & 
        - & - & - & \checkmark & $\times$ & $\times$ & 
        $\times$ & \checkmark &  - \\

\rowcolor{grey}
DeepWrinkles\cite{Lahner_2018_ECCV} & \checkmark & 4 &2 &2 & \checkmark & $\times$ & \checkmark & $\times$ & \checkmark & MSE \\

\rowcolor{grey}
MGN\cite{bhatnagar2019multi} & \checkmark & 712 & 356 & 5 & \checkmark & $\times$ & \checkmark & $\times$ & \checkmark &  - \\

\rowcolor{grey}
CAPE\cite{Ma_2020_CVPR} & \checkmark & 8 &11 & 5 & \checkmark & $\times$ & \checkmark &\checkmark & \checkmark &  L1 vert loss+L2 edge loss \\

\rowcolor{grey}
DeepFashion3D\cite{zhu2020deep} & \checkmark & 563 & - & 6 & \checkmark & $\times$ &$\times$& \checkmark & $\times$ &  - \\

\rowcolor{grey}
THUman2.0\cite{Yu_2021_CVPR} & \checkmark & - &200 & - & \checkmark & $\times$ & $\times$ & \checkmark & $\times$ &  - \\

\rowcolor{grey}
LGN\cite{Aggarwal_2022_ACCV} & \checkmark &140 &140 &5 & \checkmark & $\times$ & $\times$ &\checkmark & $\times$ &  - \\

\rowcolor{grey}
Lin et al.~\cite{Lin_2023_ICCV} &\checkmark & 
        4 & - & 3 & \checkmark & $\times$ & \times & 
        \times & \times &  -  \\

\rowcolor{grey}
\textbf{Ours} &\checkmark & \textbf{4026}
     & \textbf{2013}  &  31  & \checkmark & \checkmark  &\checkmark 
         &\checkmark  & \checkmark &  \textcolor{red}{physics-based\&CD} \\

            
\hline
\end{tabular}}

==> unused_and_backup_for_future.tex <==
\begin{table*}
\begin{center}
\scalebox{0.71}{
\begin{tabular}{l c c c c c c c c c c}
\hline

Method & 
        Dataset &\#Garment & \#Subjects & \#Categories & Real Data & Cloth design & Generation & 
        Garment-Generic &Animation & Animation Losses  \\
\hline

DRAPE\cite{guan2012drape} & \checkmark & 420 & 420 & 5 & $\times$ & $\times$ & \checkmark & $\times$ & \checkmark &  Learn from PCA \\


DeepGarment~\cite{danvevrek2017deepgarment} &\checkmark & 
        2 & 10 & 2 & $\times$ & $\times$ &\checkmark & 
        $\times$ & $\times$ &  - \\



Wang et al\cite{wang2018learning} & \checkmark & 8k & - & 3 & $\times$ & \checkmark & \checkmark &$\times$ & $\times$ &  - \\

% 3DPeople\cite{Pumarola_2019_ICCV} & \checkmark & - & 80 & - & $\times$ & $\times$ & \checkmark & \checkmark & $\times$ &  - \\



Santesteban et al.\cite{santesteban2019learning} & \checkmark & 17 & 17 & 1 & $\times$ & $\times$ & \checkmark & $\times$ & \checkmark &  Displacement loss \\

GarNet\cite{Gundogdu_2019_ICCV} & \checkmark & 1.5k & 500 & 3 & $\times$ & $\times$ & \checkmark & $\times$ & \checkmark &  L2 loss+physics-based \\


TailorNet\cite{Patel_2020_CVPR} & \checkmark & 207 & 9 & 4 & $\times$ & $\times$ & \checkmark &$\times$ & \checkmark &  L1 loss \\

Cloth3D\cite{bertiche2020cloth3d} & \checkmark & 11.3K & 8.5k & 7+ & $\times$ & $\times$ & \checkmark & \checkmark & $\times$ &  - \\


Shen et al.\cite{shen2020gan} & \checkmark & 100+ & - & 5 & $\times$ & \checkmark & \checkmark & \checkmark & $\times$ &  - \\

SMPLicit\cite{corona2021smplicit} & \checkmark & 2705k+ & - & 11 & $\times$ & $\times$ & \checkmark & \checkmark & $\times$ &  - \\

DIG\cite{Li_2022_ACCV} & $\times$ &200 &- &2 & $\times$ & $\times$ & \checkmark & \checkmark & \checkmark &  L1 loss \\

DrapeNet~\cite{De_Luigi_2023_CVPR} &\times  &
        900 & - & 5 & $\times$ & $\times$ & \checkmark & 
        \checkmark & \checkmark &  physics-based \\

HOOD~\cite{Grigorev_2023_CVPR} &\times & 
        15 & - & 7 & \times & $\times$ & \times & 
        \checkmark & \checkmark &   physics-based\\

Zhao et al.~\cite{Zhao_2023_CVPR} &\times & 
        2 & - & 2 & \times & $\times$ & \times & 
        \times & \checkmark &  L2 loss+L_{reg} \\

CLOTH4D\cite{Zou_2023_CVPR} & \checkmark & 1k & 1k & 6 & $\times$ & $\times$ & $\times$ & - & $\times$ &  - \\

ClothesNet\cite{zhou2023clothesnet} & \checkmark & 4.4k & - & 11 & $\times$ & $\times$ & $\times$ & - & $\times$ &  - \\


\rowcolor{grey}
BUFF\cite{Zhang_2017_CVPR} & \checkmark & 24 &6 &4 & \checkmark & $\times$ & $\times$ & \checkmark & $\times$ & - \\

\rowcolor{grey}
ClothCap~\cite{pons2017clothcap} &$\times$ & 
        - & - & - & \checkmark & $\times$ & $\times$ & 
        $\times$ & \checkmark &  - \\

\rowcolor{grey}
DeepWrinkles\cite{Lahner_2018_ECCV} & \checkmark & 4 &2 &2 & \checkmark & $\times$ & \checkmark & $\times$ & \checkmark & MSE \\

\rowcolor{grey}
MGN\cite{bhatnagar2019multi} & \checkmark & 712 & 356 & 5 & \checkmark & $\times$ & \checkmark & $\times$ & \checkmark &  - \\

\rowcolor{grey}
CAPE\cite{Ma_2020_CVPR} & \checkmark & 8 &11 & 5 & \checkmark & $\times$ & \checkmark &\checkmark & \checkmark &  L1 vert loss+L2 edge loss \\

\rowcolor{grey}
DeepFashion3D\cite{zhu2020deep} & \checkmark & 563 & - & 6 & \checkmark & $\times$ &$\times$& \checkmark & $\times$ &  - \\

\rowcolor{grey}
THUman2.0\cite{Yu_2021_CVPR} & \checkmark & - &200 & - & \checkmark & $\times$ & $\times$ & \checkmark & $\times$ &  - \\

\rowcolor{grey}
LGN\cite{Aggarwal_2022_ACCV} & \checkmark &140 &140 &5 & \checkmark & $\times$ & $\times$ &\checkmark & $\times$ &  - \\

\rowcolor{grey}
Lin et al.~\cite{Lin_2023_ICCV} &\checkmark & 
        4 & - & 3 & \checkmark & $\times$ & \times & 
        \times & \times &  -  \\

\rowcolor{grey}
\textbf{Ours} &\checkmark & \textbf{4026}
     & \textbf{2013}  &  31  & \checkmark & \checkmark  &\checkmark 
         &\checkmark  & \checkmark &  \textcolor{red}{physics-based\&CD} \\

            
\hline
\end{tabular}}

\end{center}
\caption{3D Garment-related methods. Grey: Real data. White:Synthetic data; \#Garment: number of different individual garments, for same garment being posed in a sequence without human shape changing we only count 1 \textcolor{red}{If we need space we can delete some rows and add a sentence ``For a full comparison between existing method we refer the reader to our supplementary material"}}
\label{table_datasets}
\end{table*}

